MR-Ben: A Meta-Reasoning Benchmark for Evaluating System-2 Thinking in LLMs

Large language models (LLMs) have shown increasing capability in problem-solving and decision-making, largely based on the step-by-step chain-of-thought reasoning processes. However, evaluating these reasoning abilities has become increasingly challenging. Existing outcome-based benchmarks are beginning to saturate, becoming less effective in tracking meaningful progress. To address this, we present a process-based benchmark MR-Ben that demands a meta-reasoning skill, where LMs are asked to locate and analyse potential errors in automatically generated reasoning steps. Our meta-reasoning paradigm is especially suited for system-2 slow thinking, mirroring the human cognitive process of carefully examining assumptions, conditions, calculations, and logic to identify mistakes.MR-Ben comprises 5,975 questions curated by human experts across a wide range of subjects, including physics, chemistry, logic, coding, and more. Through our designed metrics for assessing meta-reasoning on this benchmark, we identify interesting limitations and weaknesses of current LLMs (open-source and closed-source models). For example, with models like the o1 series from OpenAI demonstrating strong performance by effectively scrutinizing the solution space, many other state-of-the-art models fall significantly behind on MR-Ben, exposing potential shortcomings in their training strategies and inference methodologies.

==> resouce/gpt.tex <==
from openai import OpenAI


client = OpenAI(api_key='')
client.api_key='sk-6C9MuJp9tuZr62bC5157EeD2E6824fBbBd0a515462Ba4fA4'
client.base_url='https://api.gptplus5.com/v1'


content = "你是蔡徐坤吗？"


messages_few_shots = [
    {
        "role": "user",
        "content": content
    }
]


completion = client.chat.completions.create(
    model="gpt-4-1106-preview",
    messages=messages_few_shots,
    temperature=0.0

)

print(completion.choices[0].message.content)

==> sections/intro.tex <==
\begin{intro}
Pretrained with trillions of tokens and possess hundreds of billions of parameters, large language models nowadays are capable of performing complex reasoning across diverse range of tasks with near or super human performance\citep{DBLP:journals/corr/abs-2312-11805, OpenAI2022CHATGPT, ANTHROPIC2023CLAUDE}. It is therefore expected that there are heated discussions or debates within academia and social media that questions if language models are approaching human level intelligence \citep{DBLP:journals/corr/abs-2308-03762, DBLP:journals/corr/abs-2303-12712}. However, it is tricky to define what intelligence is. A direct question to ask is \textbf{Does it make sense to use the same evaluation methods toward human and language models and interpret the results indiscriminately}? \\

Given the nontransparent pretrained data corpus and instruction tuning dataset, a high-performing language model on certain benchmarks might fail to robustly generalize under new variations of the problem due to data contamination \citep{DBLP:journals/corr/abs-2311-04850, DBLP:conf/eacl/BalloccuSLD24}. One intuitive way to discriminate the `shallow' mastery of concepts or recitation of concepts from `deep' understanding or general comprehension is to ask the evaluated model to take the role of teachers instead of students \citep{zeng2024mrgsm8k}. Specifically, when tasked to give a step-by-step solutions to a given test problem, the evaluated model is only required to generate a single plausible solution out of potentially many ones. Data contamination can easily inflate the success rate of reciting possible solutions. However, by enforcing the evaluated model to adopt a role akin to the teacher to critic candidate solutions from others, the model needs to possess a comprehensive understanding of the problem to succeed in such role. Particularly, if we think of the reasoning problem as a Markov Decision Process and each step within the reasoning process is considered a state in the process, then solving the problem can be regarded as a path searching problem within a gigantic search space. To critic the candidate solutions from others, the evaluated model can no longer rely on reciting certain reasoning path, but need to actively examine the assumptions, conditions and logic within each step and collectively decide if all the steps constitutes a correct path toward the final result within the search space.\\

We follow the work of \citep{zeng2024mrgsm8k} to term the process of reason about reasoning as \textbf{Meta-Reasoning} in this work. The meta-reasoning shifts the evaluation focus from computation result (which might be generated by incorrect logic or reasoning) to the reasoning process itself. With the hope of providing a more accurate reflection of the reasoning ability of the state of the art language models, we compiled a suite of problems from diverse subjects such as Math, Coding and Logic under the Meta-Reasoning fashion we discussed above. Each question along with its various candidate solutions sampled, are meticulously annotated by a group of well-trained and selected domain experts with carefully designed cross-evaluation procedures to ensure the annotation quality. \\

Placeholder paragraph for the evaluation results and brief discussion. Placeholder paragraph for the evaluation results and brief discussion. Placeholder paragraph for the evaluation results and brief discussion. \\

In summary, the contributions of our paper are: \\
1. The compilation of a diverse and challenging benchmark that follows a novel meta-reasoning paradigm based on questions collected from existing dataset. 

2. Thorough evaluations of most popular language models from both commercial or open-source world. Our results demonstrate a significantly more differentiating ability than the benchmark that the questions were gathered from.

3. We discovered XXX relationship and uncovered some major discrepancies. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/Mr-Bean-Figure1.jpg}
    \vspace{-0.5cm}
    \caption{An overview for the \data Benchmark construction. }
    \label{fig:main}
\end{figure}





\end{intro}

==> tables/dataset.tex <==
\begin{table}
\centering
\scalebox{0.75}{
\begin{tabular}{lcccccc}
\hline
Dataset & Subject & Arithmetic & Commonsense & Logical & Symbolic & Size  \\ 
\hline
PRM800K & Math & \cmark & \xmark & \xmark & \xmark & 500$^{\dag}$ \\
BBH Mistake & Math/Logic & \cmark & \xmark & \xmark & \cmark & 2,186 \\
MR-GSM8K & Math & \cmark & \xmark & \xmark & \xmark & 3,000 \\
MR-Math & Math & \cmark & \xmark & \xmark & \xmark & 459 \\
\hline
Mr.Ben & Math/Science/Logic/Code & \cmark & \cmark & \cmark & \cmark & 10,000 \\
\hline
\end{tabular}}
% \vspace{-0cm}
\caption{Comparisons of reasoning datasets. }
\label{tab:dataset}
\end{table}

==> tables/demo.tex <==
\begin{table*}[t]
\setlength\extrarowheight{3.5pt}
% \vskip 0.15in
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrr}
\toprule
Model                                   & \multicolumn{2}{c}{\textbf{Distraction}} & \multicolumn{2}{c}{\textbf{Redefinition}} & \multicolumn{2}{c}{\textbf{Shortcut}} & \multicolumn{2}{c}{\textbf{Commonsense}} & \multicolumn{2}{c}{\textbf{Cornercase}} & \multicolumn{2}{c}{\textbf{Complex}} & \multicolumn{2}{c}{\textbf{Codesense}} & \multicolumn{2}{c}{\textbf{Total}} \\ \cline{2-17} 
                                        & $k$=1               & $k$=5              & 
$k$=1             & $k$=5             & $k$=1             & $k$=5             & $k$=1               & $k$=5              & $k$=1            & $k$=5            & $k$=1             & $k$=5           
 & $k$=1              & $k$=5             & $k$=1            & $k$=5           \\ 
 
 
    \midrule
    \multicolumn{17}{c}{\textbf{Closed-Source LLMs}}\\
    \midrule
GPT-4-1106-Preview                      & 45.0             &  58.3                  & 61.6           &      73.4             & 32.4           &          49.3         & 55.4             &      78.2              & 44.3          &             61.9     & 37.5           &         64.2         & 58.2            &         74.6          & 47.8          &     65.7            \\ 
GPT-3.5-Turbo          &  28.2 & 38.8 & 33.7 & 45.8 & 28.6 & 47.2 & 37.6 & 57.9 & 25.3 & 39.2 & 15.9 & 29.1 & 44.5 & 63.5 & 30.6 & 45.9  \\

 
    \midrule
    \multicolumn{17}{c}{\textbf{Open-Source LLMs}}\\
    \midrule
Phi 1-1.3B    &  3.0 & 9.5 & 15.7 & 25.7 & 8.8 & 15.5 & 11.2 & 18.2 & 8.3 & 18.1 & 6.9 & 11.3 & 25.7 & 34.8 & 11.4 & 19.0         \\
Phi 1.5-1.3B    &   0.9 & 3.7 & 5.5 & 12.5 & 2.9 & 8.9 & 9.0 & 17.8 & 5.4 & 11.2 & 0.6 & 2.8 & 13.9 & 24.5 & 5.5 & 11.6
        \\
Phi 2-2.7B       &    7.1 & 16.3 & 9.7 & 22.3 & 4.6 & 14.5 & 13.9 & 27.0 & 8.2 & 15.5 & 1.3 & 5.5 & 16.2 & 33.2 & 8.7 & 19.2      \\
\midrule
Mistral-7B Ins        &   3.0 & 11.1 & 7.5 & 16.8 & 2.8 & 9.5 & 7.1 & 14.4 & 9.0 & 14.7 & 0.8 & 3.4 & 13.0 & 26.3 & 6.2 & 13.7
     \\
\midrule
LLaMA2 Chat-7b       &  0.0 & 0.0 & 2.8 & 7.9 & 0.6 & 2.5 & 1.8 & 5.5 & 6.8 & 9.5 & 0.3 & 1.5 & 5.5 & 9.7 & 2.6 & 5.2
       \\
LLaMA2 Chat-13b     &  0.0 & 0.0 & 1.0 & 3.9 & 0.7 & 2.7 & 5.0 & 10.2 & 9.5 & 10.5 & 0.3 & 1.4 & 8.3 & 11.6 & 3.5 & 5.8
        \\
\midrule
CodeLLaMA-7B      &   1.4 & 6.0 & 2.6 & 10.4 & 0.7 & 3.3 & 7.0 & 18.3 & 5.7 & 11.9 & 0.3 & 1.3 & 6.5 & 15.8 & 3.4 & 9.6
         \\
CodeLLaMA-13B     &    2.2 & 9.2 & 3.1 & 12.3 & 1.6 & 7.0 & 6.0 & 17.7 & 5.6 & 14.8 & 0.8 & 3.7 & 7.7 & 19.4 & 3.9 & 12.0
        \\
CodeLLaMA-34B     & 7.1 & 20.7 & 15.4 & 34.2 & 3.8 & 13.8 & 21.2 & 43.4 & 10.5 & 23.7 & 1.5 & 6.6 & 15.0 & 33.7 & 10.6 & 25.1
       \\
\midrule
CodeLLaMA-7B Ins     &    8.2 & 20.1 & 9.7 & 17.8 & 8.5 & 15.0 & 13.2 & 23.5 & 14.7 & 19.1 & 2.2 & 7.2 & 14.2 & 25.7 & 10.1 & 18.4
         \\
CodeLLaMA-13B Ins    &    11.0 & 22.2 & 11.9 & 17.2 & 3.8 & 9.9 & 15.3 & 26.1 & 13.1 & 18.9 & 1.1 & 4.7 & 19.4 & 26.4 & 10.8 & 17.9
     \\
CodeLLaMA-34B Ins     &   6.0 & 15.5 & 11.7 & 17.3 & 7.2 & 11.3 & 23.0 & 35.8 & 9.3 & 14.4 & 0.8 & 3.5 & 17.0 & 23.7 & 10.7 & 17.4       \\
\midrule
CodeLLaMA-7B Py      &     1.2 & 5.5 & 3.0 & 11.8 & 0.6 & 2.6 & 6.9 & 18.6 & 5.4 & 11.8 & 0.4 & 2.0 & 4.9 & 12.0 & 3.2 & 9.2
    \\
CodeLLaMA-13B Py    &     1.9 & 7.4 & 6.4 & 18.5 & 1.2 & 5.2 & 9.9 & 23.5 & 6.3 & 12.9 & 0.6 & 2.9 & 9.8 & 22.1 & 5.2 & 13.2
      \\
CodeLLaMA-34B Py     &  8.0 & 24.2 & 13.6 & 32.4 & 2.5 & 10.5 & 19.6 & 43.4 & 9.9 & 20.6 & 2.0 & 9.0 & 14.2 & 32.6 & 10.0 & 24.7
 \\
\midrule
DeepSeek-1.3B     & 11.2 & 22.9 & 12.5 & 24.9 & 7.3 & 18.2 & 21.8 & 36.7 & 11.7 & 19.3 & 0.7 & 3.3 & 15.2 & 33.2 & 11.5 & 22.7
     \\
DeepSeek-6.7B      &  17.9 & 33.6 & 29.6 & 43.2 & 15.5 & 30.8 & 36.5 & 60.8 & 22.7 & 37.1 & 8.3 & 25.0 & 36.8 & 60.1 & 23.9 & 41.5     \\
DeepSeek-33B       &  \textbf{26.8} & \underline{39.2} & \textbf{35.4} & \underline{52.9} & \textbf{20.6} & \textbf{38.6} & \textbf{51.8} & \textbf{69.3} & \textbf{31.3} & \textbf{45.9} & \textbf{14.6} & \underline{34.7} & \underline{39.2} & \textbf{64.3} & \textbf{31.4} & \textbf{49.3} \\  
\midrule
WizardCoder-33B       &  \underline{25.6} & \textbf{39.9} & \underline{34.5} & \textbf{53.7} & \underline{19.8} & \underline{36.3} & \underline{48.5} & \underline{67.5} & \underline{30.6} & \underline{44.0} & \underline{14.5} & \textbf{37.7} & \textbf{39.8} & \underline{62.0} & \underline{30.5} & \underline{48.7}   \\
WizardCoder-34B Py  & 12.6 & 28.3 & 21.4 & 38.2 & 7.1 & 16.9 & 20.2 & 41.1 & 11.9 & 25.6 & 3.3 & 14.0 & 23.8 & 45.1 & 14.4 & 29.9 \\

\bottomrule
\end{tabular}
}
\caption{LLMs' performance on MHPP in terms of pass@1 and pass@5 scores.
We pinpoint top performers in open-source LLMs based on pass@1 and pass@5 scores. 
The best models are highlighted in \textbf{bold}, while those in second place are \underline{underscored}, including ties. The performance of LLMs on MHPP using greedy-search decoding can be seen in Appendix \ref{sec:greedyresult}.~\label{tab:main}}
% \vspace{-4mm}
\end{table*}

==> tables/outdated_main_table.tex <==
\begin{table*}
\caption{Evaluation Results of Models on MR-Bean: This table presents a detailed breakdown of each model’s performance evaluated under metric MR-Score across different subjects.}
\centering
\begin{tabular}{lccccccccc}
\hline
\textbf{Model} & \textbf{Method} & \textbf{Bio} &  \textbf{Phys} & \textbf{Math} & \textbf{Chem} & \textbf{Med} & \textbf{Logic} & \textbf{Coding} & \textbf{Avg} \\ 
\hline
Gemma-2b-it & 0-shot & 0.001 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 &  0.007 & 0.001 \\


Qwen-1.5-72b-Chat & 0-shot & 0.165 & 0.137 & 0.108 & 0.129 & 0.088 & 0.082 &  0.052 & 0.109  \\
Llama-2-7b-chat & 0-shot & 0.060 & 0.075 & 0.050 & 0.052 & 0.033 & 0.043 &  0.004 & 0.045  \\
Llama-3-8b-instruct & 0-shot & 0.111 & 0.149 & 0.148 & 0.128 & 0.094 & 0.096 &  0.091 & 0.117  \\
Llama-3-70b-Instruct & 0-shot & 0.199 & 0.154 & 0.150 & 0.176 & 0.146 & 0.135 &  0.282 & 0.177  \\
Claude-3-haiku & 0-shot & 0.057 & 0.033 & 0.031 & 0.065 & 0.020 & 0.012 &  0.09 & 0.044  \\
Claude-3-haiku & 1-shot & 0.058 & 0.035 & 0.031 & 0.064 & 0.020 & 0.012 &  0.00 & 0.044  \\
Mistral-Large & 0-shot & 0.222 & 0.267 & 0.243 & 0.240 & 0.159 & 0.147 &  0.211 & 0.195  \\
Mistral-Large & 1-shot & 0.280 & 0.254 & 0.282 & 0.270 & 0.193 & 0.171 &  0.214 & 0.195  \\

DeepSeek-v2-chat & 0-shot & 0.326 & 0.331 & 0.330 & 0.314 & 0.254 & 0.239 &  0.265 & 0.272 \\
GPT-3.5-turbo & 0-shot & 0.036 & 0.057 & 0.057 & 0.049 & 0.036 & 0.017 &  0.030 & 0.040  \\
GPT-3.5-turbo & 1-shot & 0.066 & 0.067 & 0.054 & 0.067 & 0.044 & 0.045 &  0.041 & 0.040  \\
GPT-4-turbo & 0-shot & 0.447 & 0.428 & 0.443 & 0.440 & 0.388 & 0.341 &  0.536 & 0.374  \\


Qwen-1.8b-chat & 0-shot & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 &  0.0 & 0.0 \\
Qwen-1.8b-chat & 1-shot & 0.0 & 0.0 & 0.001 & 0.001 & 0.0 & 0.001 &  0.0 & 0.0 \\


Phi-3-mini-4k-instruct & 0-shot & 0.120 & 0.133 & 0.115 & 0.167 & 0.115 & 0.091 & 0.089 \\
Phi-3-mini-4k-instruct & 1-shot & 0.131 & 0.108 & 0.135 & 0.144 & 0.103 & 0.046 & 0.049 \\


deepseek-llm-7b-chat & 0-shot & 0.031 & 0.047 & 0.058 & 0.033 & 0.023 & 0.029 &  0.0 & 0.032  \\
deepseek-llm-7b-chat & 1-shot & 0.049 & 0.022 & 0.055 & 0.055 & 0.025 & 0.054 & 0.007 & 0.  \\


deepseek-llm-67b-chat & 0-shot & 0.199 & 0.126 & 0.143 & 0.178 & 0.138 & 0.142 & 0.129  \\
deepseek-llm-67b-chat & 1-shot & 0.198 & 0.187 & 0.157 & 0.192 & 0.119 & 0.144 & 0.102  \\


deepseek-coder-7b-instruct-v1.5 & 0-shot & 0.125 & 0.115 & 0.100 & 0.107 & 0.102 & 0.103 &  0.017 & 0.096  \\
deepseek-coder-7b-instruct-v1.5 & 1-shot & 0.099 & 0.088 & 0.140 & 0.113 & 0.117 & 0.111 & 0.043 & 0.   \\



\hline
Gemma-2b-it & 1-shot & 0.0 & 0.0 & 0.010 & 0.0 & 0.004 & 0.002 &  0.0 & 0.002 \\
Gemma-2b-it & 2-shot & 0.001 & 0.002 & 0.007 & 0.006 & 0.007 & 0.002 &  0.0 & 0.004 \\
Gemma-2b-it & 3-shot & 0.001 & 0.003 & 0.011 & 0.001 & 0.007 & 0.003 &  0.0  & 0.004 \\
Llama-3-8b-instruct & 1-shot & 0.117 & 0.081 & 0.078 & 0.128 & 0.073 & 0.107 &  0.057 & 0.092 \\
Llama-3-8b-instruct & 2-shot & 0.097 & 0.078 & 0.111 & 0.088 & 0.064 & 0.062 &  0.024 & 0.075 \\
Llama-3-8b-instruct & 3-shot & 0.100 & 0.107 & 0.083 & 0.082 & 0.055 & 0.053 &  0.030 & 0.073 \\
Qwen-1.5-72b-Chat & 1-shot & 0.212 & 0.134 & 0.107 & 0.166 & 0.141 & 0.146 &  0.054 & 0.137 \\
Qwen-1.5-72b-Chat & 2-shot & 0.170 & 0.125 & 0.115 & 0.155 & 0.139 & 0.122 &  0.044 & 0.124 \\
Qwen-1.5-72b-Chat & 3-shot & 0.184 & 0.134 & 0.127 & 0.185 & 0.163 & 0.142 &  0.050 & 0.141 \\
Llama-3-70B-Instruct & 1-shot & 0.305 & 0.214 & 0.168 & 0.262 & 0.169 & 0.160 &  0.153 & 0.204  \\
Llama-3-70B-Instruct & 2-shot & 0.272 & 0.199 & 0.168 & 0.220 & 0.159 & 0.175 &  0.195 & 0.198  \\
Llama-3-70B-Instruct & 3-shot & 0.272 & 0.206 & 0.163 & 0.211 & 0.160 & 0.146 &  0.194 & 0.193  \\
DeepSeek-chat & 1-shot & 0.388 & 0.348 & 0.316 & 0.345 & 0.295 & 0.273 &  0.296 & 0.295 \\
DeepSeek-chat & 2-shot & 0.325 & 0.335 & 0.294 & 0.308 & 0.257 & 0.276 &  0.299 & 0.271  \\
DeepSeek-chat & 3-shot & 0.333 & 0.341 & 0.309 & 0.330 & 0.239 & 0.190 &  0.197 & 0.259  \\
GPT-4-turbo & 1-shot & 0.473 & 0.452 & 0.454 & 0.460 & 0.384 & 0.336 &  0.573 & 0.385 \\
GPT-4-turbo & 2-shot & 0.466 & 0.427 & 0.449 & 0.433 & 0.421 & 0.359 &  0.530 & 0.385 \\
GPT-4-turbo & 3-shot & 0.440 & 0.448 & 0.465 & 0.444 & 0.412 & 0.337 &  0.566 & 0.382 \\
\hline
\end{tabular}
% \label{tab:EvalResults}
\end{table*}


==> tables/stats.tex <==
\begin{table*}
\centering
\begin{tabular}{lcccc}
\hline
\textbf{Subject} & \textbf{Q-Num} & \textbf{Corr-Sols} & \textbf{Incorr-Sols}  & \textbf{Total-QS}\\ 
\hline
Logic  & 100 & 150 & 150 & 300 \\
Coding  & 100 & 150 & 150 & 300 \\
College Math  & 100 & 150 & 150 & 300 \\
College Physics  & 100 & 150 & 150 & 300 \\
College Biology  & 100 & 150 & 150 & 300 \\
College Medicine  & 200 & 300 & 300 & 600 \\
College Chemistry  & 100 & 150 & 150 & 300 \\
High School Math  & 200 & 300 & 300 & 600 \\
High School Physics  & 200 & 300 & 300 & 600 \\
High School Biology  & 200 & 300 & 300 & 600 \\
High School Chemistry  & 200 & 300 & 300 & 600 \\
Total & 1000 & 1000 & 1000 & 2000 \\
\hline
\hline
\end{tabular}
\vspace{-0cm}
\caption{This table presents the composition of our Meta-Reasoning Benchmark, where Q-Num stands for question number and Corr-Sols and Incorr-Sols stand for the number of correct/incorrect solutions sampled. The Total-QS is the total question solution pairs collected for the given subject. }
\end{table*}

==> tables/stats_full.tex <==
\begin{table*}[t]
  \centering
    % \caption{Detailed statistics of MHPP.~ \label{tab:stat}}
    % \vspace{-1em}
    %     \vskip 0.15in
   % \scalebox{0.68}{
   \begin{adjustbox}{max width=\textwidth}
  \begin{tabular}{crrrrrrrr}
    \toprule
      & Distraction & Redefinition & Shortcut & Commonsense & Cornercase & Complex & Codesense & Total \\
    \midrule
    Avg. Input Words & 238.0 & 132.5 & 125.3 & 134.6 & 137.7 & 164.8 & 118.4 & 150.2\\
    Avg. Code Lines & 13.6 & 11.7 & 4.9 & 12.5 & 13.8 & 21.5 & 7.3 & 12.2 \\
    Avg. Tests & 13.2 & 11.0 & 14.1 & 17.6 & 17.0 & 13.4 & 8.2 & 13.5 \\
    \midrule

\multirow{5}{*}{Top5 Types} 

& \multicolumn{1}{r}{Array(17\%)} & \multicolumn{1}{r}{Array(16\%)} & \multicolumn{1}{r}{Math(26\%)} & \multicolumn{1}{r}{Math(17\%)} & \multicolumn{1}{r}{Math(14\%)} & \multicolumn{1}{r}{DP(16\%)} & \multicolumn{1}{r}{String(17\%)} & \multicolumn{1}{r}{Array(15\%)} \\

 & \multicolumn{1}{r}{Hash(10\%)} & \multicolumn{1}{r}{Math(16\%)} & \multicolumn{1}{r}{Array(22\%)} & \multicolumn{1}{r}{Array(15\%)} & \multicolumn{1}{r}{Array(14\%)} & \multicolumn{1}{r}{Array(13\%)} & \multicolumn{1}{r}{Array(15\%)} & \multicolumn{1}{r}{Math(10\%)} \\
 
 & \multicolumn{1}{r}{Search(10\%)} & \multicolumn{1}{r}{DP(10\%)} & \multicolumn{1}{r}{Greedy(11\%)} & \multicolumn{1}{r}{Greedy(11\%)} & \multicolumn{1}{r}{String(11\%)} & \multicolumn{1}{r}{Stack(10\%)} & \multicolumn{1}{r}{Math(13\%)} & \multicolumn{1}{r}{String(9\%) } \\
 
  & \multicolumn{1}{r}{String(8\%)} & \multicolumn{1}{r}{Hash(8\%)} & \multicolumn{1}{r}{Sort(9\%)} & \multicolumn{1}{r}{String(9\%)} & \multicolumn{1}{r}{DP(9\%)} & \multicolumn{1}{r}{Search(9\%)} & \multicolumn{1}{r}{Hash(8\%)} & \multicolumn{1}{r}{DP(8\%)} \\
  
   & \multicolumn{1}{r}{Sort(8\%)} & \multicolumn{1}{r}{Simulation(6\%)} & \multicolumn{1}{r}{DP(7\%)} & \multicolumn{1}{r}{Geometry(7\%)} & \multicolumn{1}{r}{Search(9\%)} & \multicolumn{1}{r}{Matrix(7\%)} & \multicolumn{1}{r}{Count(8\%)} & \multicolumn{1}{r}{Sort(7\%)} \\
    

    \bottomrule
  \end{tabular}%}
  \end{adjustbox}
  % \vspace{-1em}
\caption{Detailed statistics of MHPP. Avg. Input Words represents the average number of words contained in the input, Avg. Code Lines means average number of lines in code solutions and Avg. Tests represents the average number of test cases per problem.}
\vspace{-3mm}
\end{table*}
